Fourier-Based 3D Multistage Transformer for Aberration Correction in Multicellular Specimens

High-resolution tissue imaging is often compromised by sample-induced optical aberrations that degrade resolution and contrast. While wavefront sensor-based adaptive optics (AO) can measure these aberrations, such hardware solutions are typically complex, expensive to implement, and slow when serially mapping spatially varying aberrations across large fields of view. Here, we introduce AOViFT (Adaptive Optical Vision Fourier Transformer) -- a machine learning-based aberration sensing framework built around a 3D multistage Vision Transformer that operates on Fourier domain embeddings. AOViFT infers aberrations and restores diffraction-limited performance in puncta-labeled specimens with substantially reduced computational cost, training time, and memory footprint compared to conventional architectures or real-space networks. We validated AOViFT on live gene-edited zebrafish embryos, demonstrating its ability to correct spatially varying aberrations using either a deformable mirror or post-acquisition deconvolution. By eliminating the need for the guide star and wavefront sensing hardware and simplifying the experimental workflow, AOViFT lowers technical barriers for high-resolution volumetric microscopy across diverse biological samples.

==> sections/supplementary_tables_nm.tex <==


\begin{sidewaystable}[!tp]
\caption{
\textbf{Comparisons with other ML-based AO methods}.
}
\begin{tabularx}{\textwidth}{lCCCc}
\textbf{Paper} & \makecell{\textbf{Speed}\\(time/isoplanatic patch)} & \textbf{Accuracy and Robustness} & \makecell{\textbf{Noninvasiveness}\\(photobleaching)}  & \makecell{\textbf{Code}\\\textbf{Available?}}\\
\toprule
\cite{saha2020practical} & \makecell{$\leq 1$s.} & \makecell{3D widefield PSFs.\\(Fig.~\ref{fig:comparisons-phase-retrieval-rms}--\ref{fig:comparisons-phase-retrieval-psf-rms-iterations})}  & \makecell{No extra imaging.} & \cmark \\
\midrule
\cite{rai2023deep}& \makecell{$\leq 5$s.} & \makecell{2D data.\\Samples that are sparse,\\cleared, fixed, and high SNR.}  & \makecell{1 extra (defocused) image.} & \xmark \\
\midrule
\cite{zhang2023deep} & \makecell{$\leq 1$s.} & \makecell{3D data.\\Single Molecule Light Microscopy\\data only with small aberration.\\Kalman filter needed for robustness.} & \makecell{No extra imaging.} & \cmark \\
\midrule
\cite{hu2023universal} & \makecell{Extra time needed\\to acquire M more extra images\\(M=2,4 or 2N, 4N).} & \makecell{2D data.\\Diverse sample types.\\Many manually-tuned parameters.\\ Best at 0.15--0.3 $\lambda$~RMS.\\Less accurate at 0.1--0.13 $\lambda$~RMS.}  & \makecell{Many extra images\\and motion correction\\recommended.} & \xmark \\
\midrule
\cite{kang2024coordinate} & \makecell{$\sim$5 minuets per isoplanatic\\patch of 32 megavoxels\\(200$\times$400$\times$400).} & \makecell{3D data.\\Local thresholding required\\to remove hallucinations.\\Tested with beads and\\sparse neuronal structures.\\Aberration up to 0.3 $\lambda$~RMS.\\Many manually-tuned parameters.} & \makecell{No extra imaging.} & \cmark \\
\midrule
Ours &  \makecell{$\leq 3$s (Table.~\ref{tab:performance_SH_vs_model}).} & \makecell{3D data with puncta.\\Aberration up to 1.0 $\lambda$~RMS\\(Appendix~\ref{sup:insilico}, Fig.~\ref{fig:eval-mb-rms}).\\ Confidence scores\\(Appendix~\ref{sup:confidence}).} & \makecell{No extra imaging.} & \cmark \\
\end{tabularx}
\label{tab:ao_comparisons}
\end{sidewaystable} 



\clearpage
\begin{sidewaystable}[!tp]
\caption{
\textbf{Hyperparameters for our model variants.}
A breakdown of the hyperparameters used for each stage i, 
where $p_i$ is the patch size used to tile in the input tensor, 
$n_i$ is the number of transformer layers,
$h_i$ is the number of heads for each transformer layer,
$\epsilon_i$ is the embedding size, 
and $x_i$ is the MLP size. 
Furthermore, we show the total number of trainable parameters based on the scheme used to derive each variant with the total number of transformer layers used across all stages ($n$) and the number of heads for each transformer layer ($h$).
}
\begin{tabularx}{\textwidth}{r|CCCCC|CCCCC|CC|C}
{} & \multicolumn{5}{c}{\textbf{Stage $1$}} & \multicolumn{5}{c|}{\textbf{Stage $2$}} & \multicolumn{2}{c|}{\textbf{Scheme}} & \textbf{Params} \\
\textbf{Name} & \makecell{Patch\\$p_1$} & \makecell{Layers\\$n_1$} & \makecell{Heads\\$h_1$} & \makecell{EMB\\$\epsilon_1$} & \makecell{MLP\\$x_1$} & \makecell{Patch\\$p_2$} & \makecell{Layers\\$n_2$} & \makecell{Heads\\$h_2$} & \makecell{EMB\\$\epsilon_2$} & \makecell{MLP\\$x_2$} & \makecell{Layers\\$n$} & \makecell{Heads\\$h$} & millions \\
\toprule
\textbf{Tiny  (T)} & 32 & 3 & 6 & 1024 & 4096 & 16 & 3 & 6 & 256 & 1024 & 6 & 6 & 33.9 \\
\textbf{Small (S)} & 32 & 4 & 8 & 1024 & 4096 & 16 & 4 & 8 & 256 & 1024 & 8 & 8 & 47.4 \\
\textbf{Base  (B)} & 32 & 6 & 12 & 1024 & 4096 & 16 & 6 & 12 & 256 & 1024  & 12 & 12 & 78.3 \\
\textbf{Large (L)} & 32 & 12 & 16 & 1024 & 4096 & 16 & 12 & 16 & 256 & 1024 & 24 & 16 & 171.3 \\
\textbf{Huge  (H)} & 32 & 16 & 16 & 1024 & 4096 & 16 & 16 & 16 & 256 & 1024 &  32 & 16 & 227.9 \\
\end{tabularx}
\label{tab:variants}
\end{sidewaystable} 



\clearpage
\begin{sidewaystable}[htp!]
\caption{
\textbf{Evaluation benchmark}.
}
\begin{tabularx}{\textwidth}{ccRRRRRRRRRR}
{} & {} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Testing $\lambda$ RMS}}}   & \multirow{2}{*}{\textbf{Loss}}         & \multirow{2}{*}{\textbf{Training}}  & \multirow{2}{*}{\textbf{Training}}   & \multirow{2}{*}{\textbf{Memory}}   & \multirow{2}{*}{\textbf{Throughput}}  & \multirow{2}{*}{\textbf{Latency}}     & \multirow{2}{*}{\textbf{Inference}}   & \multirow{2}{*}{\textbf{Parameters}} \\
{} & {} & \textbf{(one shot)} & \textbf{(two shot)$\downarrow$} & \textbf{($\mu$m RMS)$\downarrow$}   & \textbf{hours$\downarrow$}   & \textbf{EFLOPs$\downarrow$}      & \textbf{(GB)$\downarrow$}     & \textbf{(img/s)$\uparrow$}  & \textbf{(ms/img)$\downarrow$}    & \textbf{GFLOPs$\downarrow$}       & \textbf{(millions)$\downarrow$}  \\
\toprule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{ConvNext}}}} & \textbf{T} &  0.07 & 0.04 &          85.6$e^{-7}$ &                    37.5 &            12.9 &                     6.8 &                846 &                18.7 &   4.3 &           27.9  \\
{} & \textbf{S} &  0.04 & 0.02 &          18.8$e^{-7}$ &                    73.8 &            25.0 &                    9.4 &                648 &                32.2 &   8.4 &           49.6  \\
{} & \textbf{B} &  0.03 & 0.02 &          8.7$e^{-7}$ &                    92.0 &            44.6 &                    12.6 &                519 &                32.8 &   14.9 &            87.7  \\
{} & \textbf{L} &  0.04 & 0.02 &          7.4$e^{-7}$ &                    146.6 &            99.7 &                    19.1 &                369 &                33.3 &   33.5 &           196.4  \\
\midrule
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{ViT/16}}}} & \textbf{S}   &   0.03 & 0.02 &          28.4$e^{-7}$ &                    27.3 &            8.4 &                    2.3 &                  1326 &                15.7 &   2.8 &           71.2  \\
{} & \textbf{B}   &   0.03 & 0.02 &          4.7$e^{-7}$ &                    75.8 &            33.2 &                    5.5 &                 498 &                17.0 &   11.1 &           397.6  \\
\midrule
\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{ViT/32}}}} & \textbf{S}   &  0.04 & 0.02 &          26.8$e^{-7}$ &                    15.8 &            2.1 &                    0.9 &               2345 &                16.0 &   0.7 &           71.5  \\
{} & \textbf{B}   &  0.04 & 0.02 &          5.9$e^{-7}$ &                    28.7 &            8.4 &                    2.6 &               1557 &                16.1 &   2.8 &           398.2  \\
{} & \textbf{L}   &  0.04 & 0.02 &          2.8$e^{-7}$ &                    103.9 &            29.4 &                    9.3 &                488 &                30.6 &   9.8 &            1815.0  \\
\midrule
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Ours}}}} & \textbf{T}     &  0.04 & 0.02 &          36.3$e^{-7}$ &                    10.9 &             4.7 &                     1.4 &               2976 &                11.1 &    1.6 &           33.9  \\
{} & \textbf{S}     &  0.04 & 0.02 &          22.9$e^{-7}$ &                    13.9 &            6.3 &                    1.7 &               2522 &                13.3 &    2.1 &           47.4  \\
{} & \textbf{B}     &  0.04 & 0.02 &          11.7$e^{-7}$ &                    19.5 &            9.3 &                    2.2 &               2189 &                17.2 &   3.1 &           78.3  \\
{} & \textbf{L}     &  0.04 & 0.02 &          3.3$e^{-7}$ &                    37.0 &            18.4 &                    3.6 &                1233 &                29.0 &   6.1 &           171.3 \\
 {} & \textbf{H}     &  0.04 & 0.02 &          2.7$e^{-7}$ &                    48.2 &            24.4 &                      4.6 &                1003 &                37.7 &   8.2 &             227.9 \\
\end{tabularx}
\label{tab:benchmark}
\end{sidewaystable} 


\clearpage
\begin{table*}[!tp]
\fontsize{8pt}{8pt}\selectfont
\caption{\textbf{Residual wavefront measured using phase retrieval with widefield on an isolated bead for Fig.~\ref{fig:cells}}.}
\begin{tabularx}{\textwidth}{LCCC}
\textbf{Iteration} &    \textbf{NA} &   \makecell{\textbf{Residual WF}\\$\lambda$ RMS} & \makecell{\textbf{Residual WF}\\$\lambda$ P2V} \\
\toprule
\multicolumn{4}{c}{\textbf{Fig.~\ref{fig:cells}a}}\\
\midrule
0               &  1.00 &  0.450701 &  2.940459 \\
0               &  0.95 &  0.380205 &  2.425910 \\
0               &  0.85 &  0.292638 &  1.435171 \\
\midrule
1               &  1.00 &  0.155836 &  1.032606 \\
1               &  0.95 &  0.135578 &  0.927065 \\
1               &  0.85 &  0.096931 &  0.705702 \\
\midrule
2               &  1.00 &  0.089000 &  0.479712 \\
2               &  0.95 &  0.083749 &  0.370095 \\
2               &  0.85 &  0.077435 &  0.336847 \\
\midrule
\multicolumn{4}{c}{\textbf{Fig.~\ref{fig:cells}b}}\\
\midrule
0               &  1.00 &  0.536977 &  3.053908 \\
0               &  0.95 &  0.465103 &  2.359822 \\
0               &  0.85 &  0.425599 &  1.941650 \\
\midrule
1               &  1.00 &  0.071351 &  0.459885 \\
1               &  0.95 &  0.061207 &  0.330569 \\
1               &  0.85 &  0.054622 &  0.244614 \\
\midrule
2               &  1.00 &  0.068686 &  0.459620 \\
2               &  0.95 &  0.059220 &  0.362715 \\
2               &  0.85 &  0.048254 &  0.218788 \\
\end{tabularx}
\label{tab:cells_wavefronts}
\end{table*} 


\clearpage
\begin{sidewaystable}[!tp]
\fontsize{7pt}{7pt}\selectfont
\caption{
\textbf{Performance of SH and \model-S running on a single node with either one or four A100 GPUs}.
Benchmark for three modes of operations: default mode, smart ROI detection mode where a ROI containing diffraction-limited puncta are cropped from a scanned volume, and tiling mode. 
\model-S measurement is done on the entire 3D volume (z $\times$ y $\times$ x $\mu\text{m}^3$), whereas SH measurement is done on 3 (y $\times$ x $\mu\text{m}^2$) planes.
Total time includes initialization and setup time (\eg loading model onto each GPU), which may take between 5 and 10 seconds but is only needed at the very beginning of an imaging experiment. Since aberration measurement by SH is done serially, the SH [tile] values reported here represent the average measurement time for 288 ROIs based on the SH [default] measurement time for a single ROI. 
We also show a breakdown of the time needed for preprocessing \& embedding, smart ROI detection, and model inference time. 
}
\begin{tabularx}{\textwidth}{lCCCCCC}
\textbf{Method} & \makecell{\textbf{Predictions}\\w/ 361 rotations} & \makecell{\textbf{Preprocessing}\\\textbf{Time}} & \makecell{\textbf{ROI Detection}\\\textbf{Time}} & \makecell{\textbf{Inference}\\\textbf{Time}} & \makecell{\textbf{Total}\\\textbf{Time}} & \makecell{\textbf{GPUs}\\(A100)} \\
\toprule
\multicolumn{3}{l}{\textbf{Beads} 12.8 $\times$ 9.3 $\times$ 9.3 $\mu\text{m}^3$} & \multicolumn{4}{r}{}\\
\midrule
\model-S [default] & 1 & 2s & N/A & 3s & 8.6s & 1 \\
\model-S [default] & 361 & 2s & N/A & 3s & 9.2s & 1 \\
\model-S [default] & 361 & 2s & N/A & 9s & 16.9s & 4 \\
\midrule
\multicolumn{3}{l}{\textbf{Cells}  25.6 $\times$ 15.5 $\times$ 55.9 $\mu\text{m}^3$} & \multicolumn{4}{r}{(ROI = 12.8, 6.2, 6.2 $\mu\text{m}^3$)}\\
\model-S [default] & 1  & 3s & N/A & 3s & 8.9s  & 1 \\
\model-S [default] & 361  & 3s & N/A & 3s & 9.3s  & 1 \\
\model-S [default] & 361  & 3s & N/A & 9s & 18.1s  & 4 \\
\model-S [roi-1] & 361  & 3s & 3s & 9s & 25.3s & 4 \\
\model-S [roi-10] & 3610 & 6s & 9s & 15s & 40.6s & 4 \\
\midrule
\multicolumn{3}{l}{\textbf{Zebrafish small FOV} 12.8 $\times$ 12.4 $\times$ 12.4 $\mu\text{m}^3$} & \multicolumn{4}{r}{(ROI = 12.8, 6.2, 6.2 $\mu\text{m}^3$)}\\
\midrule
SH [default] & 1 & N/A & N/A & N/A &  5.1s & N/A \\
\model-S [default] & 1  & 3s & N/A & 3s &  8.8s & 1 \\
\model-S [default] & 361  & 3s & N/A & 3s &  9.2s & 1 \\
\model-S [default] & 361  & 3s & N/A & 9s &  17.0s & 4 \\
\model-S [roi-1] & 361 & 3s & 3s & 9s & 23.7s  & 4 \\
\model-S [roi-10] & 3610 & 6s  & 9s & 15s & 38.9s & 4 \\
\midrule
\multicolumn{3}{l}{\textbf{Zebrafish large FOV} 12.8 $\times$ 49.7 $\times$ 223.5 $\mu\text{m}^3$} & \multicolumn{4}{r}{(TILE = 12.8, 9.3, 9.3 $\mu\text{m}^3$)}\\
\midrule
SH [tile]  & 288 tiles & N/A & N/A & N/A &  1,468.8s & N/A \\
\model-S [tile]  & \makecell{103,968\\(288 tiles  $\times$  361)} & 30.6s & N/A & 91.4s &  139.8s & 4 \\
\end{tabularx}
\label{tab:performance_SH_vs_model}
\end{sidewaystable} 


\clearpage
\begin{sidewaystable}[htp!]
\centering \scriptsize
\caption{
\textbf{Light sheet specifications}. \textit{MBSq-35} LLS excitation profile was used for simulating training data.
}
\begin{tabularx}{\textwidth}{LlCCCCCCC}
\textbf{Name} & \textbf{Lattice type} & \textbf{$\text{NA}_{lattice}$} & \textbf{$\text{NA}_{exc}$} & \textbf{$\text{NA}_{sinc}$} & \textbf{$\text{NA}_{annulus}$} & \textbf{$\sigma_{\text{NA}}$} & \textbf{FWHM} & \textbf{Crop} \\
\toprule
\textbf{MBSq-30}     & Multi-Bessel square LLS                    & 0.30 & - & - & 0.375/0.225 & 0.10 & 48.5 & - \\
\textbf{MBSq-35}     & Multi-Bessel square LLS                    & 0.35 & - & - & 0.40/0.30 & 0.10 & - & - \\
\textbf{MBSq-50}     & Multi-Bessel square LLS                    & 0.50 & - & - & 0.40/0.30 & 0.10 & - & - \\
\textbf{Sinc}        & Simulated by swept lateral standing wave   & - & 0.32 & 0.24 & 0.40/0.20 & - & 51.5 & - \\
\textbf{Gaussian}    & Simulated by swept lateral standing wave   & - & 0.21 & - & 0.40/0.20 & 0.21 & 51.0 & 0.1 \\
\end{tabularx}
\label{tab:lightsheets}
\end{sidewaystable} 





\clearpage
\begin{sidewaystable}[htp!]
\fontsize{6pt}{6pt}\selectfont
\caption{
\textbf{Imaging configuration.} All data was collected using \textit{MBSq-35} light sheet described in Supplementary Table~\ref{tab:lightsheets}.
}
\begin{tabularx}{\textwidth}{lCCCC}
\textbf{Figure | Scan type} & \makecell{\textbf{Voxel size}\\(x, y, z)} & \makecell{\textbf{Volume size}\\(x, y, z)} & \makecell{\textbf{Excitation}\\\textbf{wavelength}} & \makecell{\textbf{Camera}\\\textbf{Exposure}} \\
\toprule
\textbf{Fig.~\ref{fig:cells}} | Widefield Scan & 97, 97, 100 nm & 96, 96, 128  & 488 nm  & 50 ms \\
\textbf{Fig.~\ref{fig:cells}} | Cell Scan & 97, 97, 200 nm & 160, 576, 128  & 488 nm, 560 nm  & 50 ms \\
\midrule
\textbf{Fig.~\ref{fig:fish_online}a} | No AO Full Chip Scan & 97, 97, 200 nm & 2304, 2304, 64  & 488 nm , 560 nm  & 50 ms \\
\midrule
\textbf{Fig.~\ref{fig:fish_online}b} | No AO Scan 1 & 97, 97, 200 nm & 128, 128, 64  & 488 nm, 560 nm  & 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}b} | DSH 1 & 0.1, 6.2, 6.3 um & 125, 3, 3  & 920 nm  & 500 ms \\
\textbf{Fig.~\ref{fig:fish_online}b} | DSH 2 & 0.1, 6.2, 6.3 um & 125, 3, 3  & 920 nm  & 400 ms \\
\textbf{Fig.~\ref{fig:fish_online}b} | DSH 3 & 0.1, 6.2, 6.3 um & 125, 3, 3  & 920 nm  & 400 ms \\
\textbf{Fig.~\ref{fig:fish_online}b} | SH AO Scan & 97, 97, 200 nm & 128, 128, 64  & 488 nm , 560 nm  & 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}b} | No AO Scan 2 & 97, 97, 200 nm & 128, 128, 64  & 488 nm , 560 nm  & 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}b} | AOViFT Iter 1 Scan & 97, 97, 200 nm & 128, 128, 64  & 488 nm , 560 nm  & 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}b} | AOViFT Iter 2 Scan & 97, 97, 200 nm & 128, 128, 64  & 488 nm , 560 nm  & 50 ms \\
\midrule
\textbf{Fig.~\ref{fig:fish_online}c} | No AO Full Chip Scan & 97, 97, 200 nm & 2304, 2304, 64 & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | No AO Scan 1 & 97, 97, 200 nm & 128, 128, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | DSH 1 & 0.1, 6.2, 6.3 um & 125, 3, 3  & 920 nm & 500 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | DSH 2 & 0.1, 6.2, 6.3 um & 125, 3, 3  & 920 nm  & 500 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | DSH 3 & 0.1, 6.2, 6.3 um & 125, 3, 3  & 920 nm  & 500 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | SH AO Scan & 97, 97, 200 nm & 128, 128, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | No AO Scan 2 & 97, 97, 200 nm & 128, 128, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | AOViFT Iter 1 Scan & 97, 97, 200 nm & 128, 128, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | AOViFT Iter 2 Scan & 97, 97, 200 nm & 128, 128, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:fish_online}c} | AOViFT Full Chip Scan & 97, 97, 200 nm & 2304, 2304, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\midrule
\textbf{Fig.~\ref{fig:fish_offline}b} | AOViFT Full Chip Scan & 97, 97, 200 nm & 2304, 2304, 64  & 488 nm & 50 ms \\
\midrule
\textbf{Fig.~\ref{fig:fish_offline}d} | AOViFT Full Chip Scan & 97, 97, 200 nm & 2304, 2304, 64  & 560 nm & 50 ms \\
\midrule
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | No AO Full Chip Scan & 97, 97, 200 nm & 2304, 2304, 64 & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | No AO Scan 1 & 97, 97, 200 nm & 256, 256, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | DSH 1 & 0.1, 6.2, 6.2 um & 125, 3, 3  & 920 nm & 400 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | DSH 2 & 0.1, 6.2, 6.2 um & 125, 3, 3  & 920 nm  & 400 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | DSH 3 & 0.1, 6.2, 6.2 um & 125, 3, 3  & 920 nm  & 400 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | SH AO Scan & 97, 97, 200 nm & 256, 256, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | No AO Scan 2 & 97, 97, 200 nm & 256, 256, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | AOViFT Iter 1 Scan & 97, 97, 200 nm & 256, 256, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\textbf{Fig.~\ref{fig:Figure4_SI1}--\ref{fig:Figure4_SI2}} | AOViFT Iter 2 Scan & 97, 97, 200 nm & 256, 256, 64  & 488 nm, 560 nm & 50 ms, 50 ms \\
\end{tabularx}
\label{tab:imaging_configuration}
\end{sidewaystable}





\clearpage
\begin{table*}[htp!]
\fontsize{8pt}{8pt}\selectfont
\caption{
\textbf{Training configuration}.
}
\begin{tabularx}{\textwidth}{L|C}
\toprule
\multicolumn{2}{c}{\textbf{Optical configuration}} \\
\midrule
Lattice type                & \textit{MBSq-35} (Supplementary Table~\ref{tab:lightsheets}) \\
$\text{NA}_{exc}$           & 0.35 \\
$\text{NA}_{annulus}$       & 0.4/0.3 \\
$\text{NA}_{detection}$     & 1.0 \\
$\sigma_{\text{NA}}$        & 0.10 \\
Refractive index            & 1.33 \\
Excitation wavelength       & 488 nm \\
Detection wavelength ($\lambda$)      & 510 nm \\
Voxel size                  & $200^Z, 125^Y, 125^X$ nm \\
\midrule
\multicolumn{2}{c}{\textbf{Training Dataset}} \\
\toprule
Dataset size                & 2M synthetic samples \\
Number of beads             & $b \in \{1 \to 5\}$ \\
Bead size                   & $\text{FWHM} \in \{100, 200, 300, 400\}nm$ \\
Mode distribution(s)        & $\mathcal{D} \in$ \{Single, Bimodal, Powerlaw, Dirichlet\} \\ 
Mode weighting ($Z_n^m$)    & Uniform $n \in \{2\to4\}$ \& linear decay $n \in \{4\to10\}$ \wrt $m$ \\ 
Magnitude range             & $a \in \{0\to0.3\}\mu$m $\Longleftrightarrow$ $a \in \{0\to5\}\lambda$ \\
Image size                  & $64^Z, 64^Y, 64^X$ voxels $\Longleftrightarrow$ $12.8^Z, 8^Y, 8^X$ $\mu$m \\
\midrule
\multicolumn{2}{c}{\textbf{Hyperparameters}} \\
\toprule
Batch size                  & 4096      \\
Loss                        & MSE       \\
Optimizer                   & AdamW~\cite{loshchilov2018decoupled} \\
Layerwise decay             & LAMB~\cite{you2020large} \\ 
Momentum $\beta_1$          & 0.9        \\
Momentum $\beta_2$          & 0.99       \\
Initial learning rate (LR)  & 0.0001     \\
Weight decay                & 0.001      \\
\midrule
\multicolumn{2}{c}{\textbf{Training schedulers}} \\
\toprule
Total epochs                & 500           \\
Warmup epochs               & 25            \\
Warmup scheduler            & Linear        \\
Learning rate decay         & Cosine~\cite{loshchilov2016sgdr} \\
\bottomrule
\end{tabularx}
\label{tab:training_config}
\end{table*} 

\clearpage



==> settings.tex <==
\usepackage{seqsplit}
\usepackage{titletoc}

%% links
\usepackage{url}
%% url style
\urlstyle{same}

%% allow hyphenation for urls with long many-hyphenated strings
\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
  allcolors=skyblue,
  urlcolor=gray,
  citecolor=skyblue,
  pdfborder={0 0 0},
  breaklinks=true,
}
\RequirePackage{hyperxmp}

%% captions should have label bold, description normal (up to you to boldface the caption tile line).
\usepackage[labelfont=bf,textfont=md]{caption}

%% build papers out of todo lists
\usepackage{color}
\usepackage{xcolor}

\definecolor{skyblue}{HTML}{1569C7}
\definecolor{gray}{HTML}{808080}
\definecolor{firebrick}{HTML}{B22222}
\definecolor{seagreen}{HTML}{2E8B57}




\usepackage{graphicx}
\usepackage{epsfig,verbatim,enumerate}


\usepackage{tabularx}
\usepackage{multirow, makecell}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1.5}


\usepackage{mathtools}
\usepackage{amsfonts}

\newcommand{\avg}[1]{\left\langle#1\right\rangle}
\newcommand{\tavg}[1]{\langle#1\rangle}

\newcommand{\LavgHa}[2]{\tavg{L_{#1,#2}}}
\newcommand{\LavgHaN}[2]{\tavg{L_{#1,#2}}}
\newcommand{\Lavg}{\tavg{L}}

\newcommand{\sindex}[1]{}
\newcommand{\nindex}[1]{}

\newcommand{\www}[1]{\url{#1}}
\newcommand{\req}[1]{(\ref{#1})}
\newcommand{\Req}[1]{Eq.~(\ref{#1})}
\newcommand{\etal}{\textit{et al}.}
\newcommand{\etc}{\textit{etc}} 
\newcommand{\ie}{i.e.,~}  % grammar rules say no italics
\newcommand{\eg}{e.g.,~}  % grammar rules say no italics
\newcommand{\wrt}{\textit{w}.\textit{r}.\textit{t}.~} 

% lettrines
\usepackage{lettrine}

\newcommand{\tbf}{\textbf}
\newcommand{\tit}{\textit}

%% differential equations and integrals
\newcommand{\dee}[1]{\textnormal{d}#1}
\newcommand{\pdiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdiffsq}[2]{\frac{\partial^2 #1}{{\partial #2}^2}}
\newcommand{\diff}[2]{\frac{{\rm d}#1}{{\rm d}#2}}
\newcommand{\diffsq}[2]{\frac{{\rm d}^{2}#1}{{\rm d} {#2}^2}}
\newcommand{\tdiff}[2]{\textnormal{d} #1/\textnormal{d} #2}
\newcommand{\tdiffsq}[2]{\textnormal{d}^{2} #1/\textnormal{d} {#2}^2}
\newcommand{\tpdiff}[2]{\partial #1/\partial #2}
\newcommand{\tpdiffsq}[2]{\partial^2 #1/\partial {#2}^2}
\newcommand{\postdee}[1]{\,\textnormal{d}#1}


\usepackage{enumitem}

\newcommand{\Prob}[1]{{\rm Pr}\left(#1\right)}

%% contagion

% \newcommand{\kstar}{d^{\ast}}
% \newcommand{\kstari}{k_i^\ast}
\newcommand{\kstar}{d^\ast}
\newcommand{\kstari}{d_i^\ast}

\newcommand{\dstar}{d^\ast}
\newcommand{\dstari}{d_i^\ast}

\newcommand{\phifix}{{\phi^{\ast}}}
\newcommand{\phifixc}{{\phi_c^{\ast}}}
\newcommand{\phifixb}{{\phi_b^{\ast}}}

\newcommand{\phiiactive}{\phi_{i,t}}

\newcommand{\phiiup}{{\phi_{i,\rm on}}}
\newcommand{\phiidown}{{\phi_{i,\rm off}}}

\newcommand{\Gfun}{G}

\newcommand{\dstardist}{g}
\newcommand{\dosedist}{f}
\newcommand{\dosedistk}{f^{k\star}}

% chaotic contagion
\newcommand{\edgeinfprob}{\rho}
\newcommand{\nodeinfprob}{\phi}

\newcommand{\avgdegree}{k_{\rm avg}}

\newcommand{\stateA}{S_{0}}
\newcommand{\stateB}{S_{1}}

\newcommand{\lcce}{H}

%% \newcommand{\effectivecount}{f_{\textnormal{eff}}}

\newcommand{\effectivecount}{f_{q,\textnormal{exp}}}
\newcommand{\effectivecountq}[1]{f_{#1,\textnormal{exp}}}

\newcommand{\simonrho}{\rho}
\newcommand{\zipfexponent}{\alpha}

\newcommand{\partitionprob}{q}
\newcommand{\partitiontype}[1]{$\partitionprob$$=$$#1$}

\newcommand{\onehalf}{\frac{1}{2}}
\newcommand{\onequarter}{\frac{1}{4}}

\newcommand{\clgamma}{\hat{\zipfexponent}}
\newcommand{\xmin}{r_{\textnormal{max}}}
\newcommand{\kstat}{D}
\newcommand{\clp}{\textnormal{$p$-value}}
\newcommand{\sigamma}{1-\simonrho}


\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\tcn}[2]{\color[named]{#1}{#2}}



\newcommand{\addcite}{\textcolor{firebrick}{\{CITE\}}}
\newcommand{\paragraphnutshell}[1]{\noindent\textcolor{firebrick}{{Paragraph: #1}}}




\newcommand{\model}{\textsc{AOViFT}}
\def\els@aparagraph[#1]#2{\elsparagraph[#1]{#2.}}


\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


